Statistical Inference for High-Dimensional Robust Linear Regression Models via Recursive Online-Score Estimation

This paper introduces a novel framework for estimation and inference in penalized M-estimators applied to robust high-dimensional linear regression models. Traditional methods for high-dimensional statistical inference, which predominantly rely on convex likelihood-based approaches, struggle to address the nonconvexity inherent in penalized M-estimation with nonconvex objective functions. Our proposed method extends the recursive online score estimation (ROSE) framework of Shi et al. (2021) to robust high-dimensional settings by developing a recursive score equation based on penalized M-estimation, explicitly addressing nonconvexity. We establish the statistical consistency and asymptotic normality of the resulting estimator, providing a rigorous foundation for valid inference in robust high-dimensional regression. The effectiveness of our method is demonstrated through simulation studies and a real-world application, showcasing its superior performance compared to existing approaches.

==> macros.tex <==
\def\boe{\begin{enumerate}}
\def\eoe{\end{enumerate}}
\def\dom{\mathrm{dom}}
%\newtheorem{proposition}{{\bf Proposition}}
%\newtheorem{lemma}{{\bf Lemma}}
%\newtheorem{corollary}{{\bf Corollary}}
%\newtheorem{assumption}{{\bf Assumption}}
%\newtheorem{definition}{{\bf Definition}}
%\newtheorem{theorem}{{\bf Theorem}}
%\newtheorem{conjecture}{{\bf Conjecture}}
%\newtheorem{example}{{\bf Example}}
%\newtheorem{problem}{{\bf Problem}}
\newcommand\ca[1]{{\cal{#1}}}
\newcommand\lo[1]{_{\nano{#1}}}
\newcommand\hi[1]{^{\nano{#1}}}
\def\fsave{\mathrm{f\mbox{-}SAVE}}
\def\circtauyt{\topcirc \tau \lo Y \phantom{A}\hspace{-.17in}\trans }
\def\diag{{\mathrm{diag}}}
%\renewcommand{\thesubsection}{\arabic{subsection}}
\renewcommand{\thesubsubsection}{\arabic{subsection}.\arabic{subsubsection}}
\def\cid{\stackrel{\mbox{\tiny $\cal D$}}\longrightarrow}
\def\argmin{\mathrm{argmin}}
\def\Range{\mathrm{Range}}
\def\Span{\mathrm{Span}}
\def\proof{\noindent {\sc Proof. }}
\def\Sigmaxx{\Sigma_{\mbox{\tiny $X\!X$}}}
\def\Sigmaxy{\Sigma_{\mbox{\tiny $X\!Y$}}}
\def\Sigmayx{\Sigma_{\mbox{\tiny $Y\!X$}}}
\def\Sigmayh{\Sigma_{\mbox{\tiny $Y\!H$}}}
\def\Sigmahh{\Sigma_{\mbox{\tiny $H\!H$}}}
\def\Sigmahy{\Sigma_{\mbox{\tiny $H\!Y$}}}
\def\Sigmayy{\Sigma_{\mbox{\tiny $Y\!Y$}}}
\def\cip{\stackrel{\mbox{\tiny $P$}}\rightarrow}
\def\As{{\mbox{\tiny $A$}}}
\def\Ss{{\mbox{\tiny $S$}}}
\def\Es{{\mbox{\tiny $E$}}}
\def\E{\mathbb{E}}
\def\R{\mathbb R}
\def\S{\mathbb S}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal{H}}}
\def\HT{\H \lo T}
\def\HX{\H \lo X}
\def\HY{\H \lo Y}
%\def\M{{\cal M}}
\def\L{{\cal L}}
\def\M{\mathfrak M}
\def\N{{\mathfrak {N}}}
\def\S{{\mathfrak{S}}}
\def\PCA{{\mbox{\tiny $\mathrm{PC}$}}}
\def\RR{{\mbox{\tiny $\mathrm{RR}$}}}
\def\given{| \,}
\def\central{{\mathfrak{S}_{\nano Y|X}}}
\def\cfield{{\G_{\nano Y|X}}}
\def\tsum{\textstyle{\sum}}
\def\Xb{\boldsymbol X}
\def\trans{^{\mbox{\tiny{\sf  T}}}}
\def\Yb{\boldsymbol Y}
\def\eqdis{\stackrel{\mbox{\tiny $\cal D$}}{=}}
\def\half{^{\mbox{\tiny $\frac{1}{2}$}}}
\def\mhalf{^{\mbox{\tiny $-\frac{1}{2}$}}}
\def\inv{^{\mbox{\tiny $-1$}}}
\def\thetabfs{{\mbox{\tiny $\thetabf$}}}
\def\Xbfs{{\mbox{\tiny $\Xbf$}}}
\def\var{\mathrm{var}}
\def\cov{\mathrm{cov}}
%\newcommand{\indep}{\;\, \rule[0em]{.03em}{.65em} \hspace{-.45em}
%\rule[-.05em]{.65em}{.03em} \hspace{-.45em}
%\rule[0em]{.03em}{.65em}\;\,}


\newcommand{\indep}{\;\, \rule[0em]{.03em}{.65em} \hspace{-.41em}
\rule[-.02em]{.65em}{.03em} \hspace{-.41em}
\rule[0em]{.03em}{.65em}\;\,}


\def\subshat{\, \, \hat {\!\!\stens S}}
\def\shat{\ \hat{\!\! \sten S}}
\def\stenhat#1{\ \, \hat{\!\!\!  #1}}
\def\tr{\mathrm{tr}}
\def\vec{\mathrm{vec}}
\def\mat{\mathrm{mat}}
\def\sign{\mathrm{sign}}
\def\eop{\hfill $\Box$ \\
}
\def\trans{^{\mbox{\tiny{\sf T}}}}
\def\Xs{{\mbox{\tiny $X$}}}
\def\cid{\stackrel{\mbox{\tiny $\cal D$}}\rightarrow}
\def\iff{\Leftrightarrow}
\def\gpc{{\cal G}}
\def\dy{D_{{\mbox{\tiny $Y$}}}}
\def\du{D_{{\mbox{\tiny $U$}}}}
\def\kappax{\kappa_{\mbox{\tiny $X$}}}
\def\kappat{\kappa_{\mbox{\tiny $T$}}}
\def\kappay{\kappa_{\mbox{\tiny $Y$}}}
\def\Xsmall{\mbox{\tiny $X$}}
\def\Ysmall{\mbox{\tiny $Y$}}
\def\yygx{{\mbox{\tiny $YY|X$}}}
\def\xxsub{{\mbox{\tiny $XX$}}}
\def\yysub{{\mbox{\tiny $YY$}}}
\def\xysub{{\mbox{\tiny $XY$}}}
\def\yxsub{{\mbox{\tiny $YX$}}}
\def\Psub{{\mbox{\tiny $P$}}}
\def\ali{&\,}
\def\card{{\mathrm{card}}}
\def\spc{{\cal S}}
\def\ran{\mathrm{ran}}
\def\XYsub{{\mbox{\tiny $XY$}}}
\def\Xsub{{\mbox{\tiny $X$}}}
\def\Ysub{{\mbox{\tiny $Y$}}}
\def\central{\sten S \lo {Y|X}}
\def\quo{^\circ}
\def\of{{\nano {\circ}}}
\def\nano{\scriptscriptstyle}
\def\scirc{{\mbox{\tiny $\circ$}}}
\def\coxx{\Sigma_{\nano XX}}
\def\coxy{\Sigma_{\nano XY}}
\def\coyx{\Sigma_{\nano YX}}
\def\coyy{\Sigma_{\nano YY}}
\def\half{^{\nano 1/2}}
\def\nhalf{^{\nano -1/2}}
\def\rxy{R_{\nano XY}}
\def\ryx{R_{\nano YX}}
\def\hx{{\H_{\nano X}}}
\def\hy{{\H_{\nano Y}}}
\def\ltwox{{L_2(P_{\nano X})}}
\def\ltwoy{{L_2(P_{\nano Y})}}
\def\mean{\overline}
\def\cltwox{\mathrm{cl}_\ltwox}
\def\chx{\mathrm{cl}_\hx}
\def\equal{&=\, }
\def\real{{\mathbb R}}
\def\ddo{{$\ddot{\mbox{o}}$}}
\def\ddu{{$\ddot{\mbox{u}}$}}
\def\complete{\mathfrak{C}_{\nano Y|X}}
\def\completeoc{\mathfrak{C}_{\nano Y|X}\oc}
\def\tint{\textstyle{\int}}
\def\ka{\kappa}
\def\cenclass{\mathfrak{S} \lo {Y|X}}
\newcommand\oop[4]{#1 \lo {{\uppercase{#2}}({\uppercase{#3}} \otimes {\uppercase{#4}})}}
\def\oc{^{\nano \perp}}
\def\X{\cal{X}}
\def\Y{\cal{Y}}
\def\L2T{L \lo 2 (T)}
\def\L2TX{L \lo 2 (T\lo X)}
\def\L2TX{L \lo 2 (T\lo Y)}
\def\tsum{\textstyle{\sum}}
\def\ali{&\,}
\def\spn{{\rm{span}}}
\def\ali{&\,}
\def\adj{\hi *}
\def\eod{\end{document}}
\def\mpinv{\hi {\dagger}}
\def\shortbar{\rule[-.0em]{.04em}{.15em}}
\def\bbar{\mbox{\raisebox{-.05em}{$\,\overset{\overset{\shortbar}{\shortbar}}{\shortbar}\,$}}}
\newcommand\remind[1]{{\color{red}{{#1}}}}
%\def\red#1{{\color{red}{{#1}}}}
%\def\blue#1{{\color{blue}{{#1}}}}
\newcommand\ask[1]{{\color{blue}{{#1}}}}

\newcommand{\lbing}{\;\, \rule[0em]{.13em}{1.5em}}

%\tikzset
%{
%    x=2cm,% default value is 1cm.
%    y=3cm,% default value is 1cm.
%}

\def\lbing{
\!\raisebox{-2.3pt}{ \tikz[x=2.5pt,y=2.6pt]{\draw[line width=0.4pt](-1+4.8,-1)--(0+4.8,-2);\draw[line width=0.4pt](-1+4.8,1)--(0+4.8,2);\draw[line width=0.4pt](-1+4.8,1-2)--(-1+4.8,0+1);}}\hspace{0pt}}
\def\rbing{\!\!
\raisebox{-2.3pt}{ \tikz[x=2.5pt,y=2.6pt]{\draw[line width=0.4pt](-1-0.8,-2)--(0-0.8,-1);\draw[line width=0.4pt](-1-0.8,2)--(0-0.8,1);\draw[line width=0.4pt](0-0.8,-1)--(0-0.8,1);}}}


\def\cran{{\overline{{\rm{ran}}}}}
\def\dom{\mathrm{dom}}




\def\topcirc#1{\overset{\nano \circ}{#1}}
\newcommand{\red}[1]{{\leavevmode\color{red}{#1}}}
\newcommand{\blue}[1]{{\leavevmode\color{blue}{#1}}}
\newcommand{\magenta}[1]{{\leavevmode\color{magenta}{#1}}}
\newcommand{\cyan}[1]{{\leavevmode\color{cyan}{#1}}}
\newcommand{\green}[1]{{\leavevmode\color{green}{#1}}}
\newcommand{\brown}[1]{{\leavevmode\color{Brown}{#1}}}
\newcommand{\olivegreen}[1]{{\leavevmode\color{OliveGreen}{#1}}}
\newcommand{\mahogany}[1]{{\leavevmode\color{Mahogany}{#1}}}
\newcommand{\navyblue}[1]{{\leavevmode\color{NavyBlue}{#1}}}
\newcommand{\mulberry}[1]{{\leavevmode\color{Mulberry}{#1}}}
\newcommand{\redorange}[1]{{\leavevmode\color{RedOrange}{#1}}}
\def\card{{\mathrm{card}}}
\newcommand{\skyblue}[1]{{\leavevmode\color{SkyBlue}{#1}}}
\newcommand{\salmon}[1]{{\leavevmode\color{Salmon}{#1}}}
\def\loo#1{_{\nano{\mathrm{\uppercase{#1}}}}}


%\Large
\newfont{\rsfsten}{rsfs10 scaled 1100}
\newfont{\rsfstena}{rsfs10 scaled 800}
%\newfont{\rsfsten}{rsfs10 scaled 1300}
%\newfont{\rsfstena}{rsfs10 scaled 800}
\newfont{\rsfstenb}{rsfs10 scaled 500}
\newcommand{\sten}[1]{\mbox{\rsfsten #1}\,}
\newcommand{\stens}[1]{\mbox{\rsfstena #1}\,}
\newcommand{\stent}[1]{\mbox{\rsfstenb #1}}



\def\iff{\Leftrightarrow}

\def\dom{{\mathrm{dom}}}
\def\imply{\Rightarrow}
\def\central{\sten S \lo {Y|X}}





\def\central{\sten S \lo {Y|X}}
\def\hatcentral{\stenhat {\sten S} \lo {Y|X}}
\def\shortbar{\rule[-.0em]{.04em}{.15em}}
\def\bbar{\mbox{\raisebox{-.05em}{$\,\overset{\overset{\shortbar}{\shortbar}}{\shortbar}\,$}}}







==> misc.tex <==

\usepackage{bbm}
\usepackage{mathrsfs}
 %\usepackage{mathbbold
\usepackage{amsfonts}
\usepackage{float}
\usepackage{amsthm}
\usepackage{epsfig,rotating}
\usepackage{amssymb,amsmath}
\usepackage{latexsym}
\usepackage{appendix}
\usepackage{graphicx,subfigure}
\usepackage{multirow}
\usepackage{color}
\usepackage{booktabs}
\usepackage[round, authoryear]{natbib}
\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{subfigure}
\usepackage{natbib,float}
\usepackage{comment}



\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\def\ba{\boldsymbol{a}}
\def\bb{\boldsymbol{b}}
\def\bB{\boldsymbol{B}}
\def\bx{\boldsymbol{x}}
\def\bX{\boldsymbol{X}}
\def\bI{\boldsymbol{I}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}
\def\bZ{\boldsymbol{Z}}
\def\bw{\boldsymbol{\omega}}

\def\bW{\boldsymbol{W}}
\def\bu{\boldsymbol{u}}
\def\bU{\boldsymbol{U}}
\def\bv{\boldsymbol{v}}
\def\bP{\boldsymbol{P}}
\def\bp{\boldsymbol{p}}
\def\bq{\boldsymbol{q}}
\def\btheta{\boldsymbol{\theta}}
\def\bTheta{\boldsymbol{\Theta}}
\def\bbeta{\boldsymbol{\beta}}
\def\bbetat{\widetilde{\boldsymbol{\beta}}}
\def\bmu{\boldsymbol{\mu}}
\def\beda{\boldsymbol{\eta}}
\def\bSigma{\boldsymbol{\Sigma}}
\def\b1{\boldsymbol{1}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\setlength{\textheight}{8.5in} \setlength{\textwidth}{6.0in}
\setlength{\evensidemargin}{0.2in} \setlength{\oddsidemargin}{0.2in}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bali}{\begin{align*}}
\newcommand{\eali}{\end{align*}}
\newcommand{\lbl}{\label}
\newcommand{\eq}[1]{$(\ref{#1})$}
\newcommand{\bS}{\boldsymbol{\Sigma}}


\newcommand{\ml}{\mathcal}
\newcommand{\lth}{\Lambda'(\theta)}
\newcommand{\bs}{\backslash}
\newcommand{\mn}{|\!|\!|}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lra}{\Leftrightarrow}
\newcommand{\M}{\mathcal{M}}
\newcommand{\bbx}{{\bf {x}}}
\newcommand{\bby}{{\bf {y}}}
\newcommand{\bbz}{{\bf {z}}}
\newcommand{\bbv}{{\bf {v}}}
\newcommand{\bbu}{{\bf {u}}}
\newcommand{\bbw}{{\bf{w}}}
\newcommand{\bbX}{{\bf {X}}}
\newcommand{\bbY}{{\bf {Y}}}
\newcommand{\bbS}{{\bf S}}
\newcommand{\bbZ}{{\bf Z}}
\newcommand{\bbR}{{\bf R}}
\newcommand{\bbA}{{\bf A}}
\newcommand{\bbB}{{\bf B}}
\newcommand{\bbC}{{\bf C}}
\newcommand{\bbQ}{{\bf Q}}
\newcommand{\bbW}{{\bf W}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mE}{\mathbb{E}}
\newcommand{\mP}{\mathbb{P}}
\newcommand{\mK}{\mathbb{K}}
\newcommand{\mC}{\mathbb{C}}
\newcommand{\mX}{\mathbb{X}}
\newcommand{\mS}{\mathbb{S}}
\newcommand{\gS}{{\Sigma}}
\newcommand{\prk}{{R(\boldsymbol{\beta})}}
\newcommand{\erk}{{\widehat{R}_n(\boldsymbol{\beta})}}
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\hbeta}{\boldsymbol{\hat\beta}}
\newcommand{\tbeta}{\boldsymbol{\tilde\beta}}
\newcommand{\tlambda}{\tilde\lambda}
\newcommand{\aset}{\mathcal{A}}
\newcommand{\hm}{\mathit{h}_{\max}}
\newcommand{\gbeta}{G(\boldsymbol{\beta})}
\newcommand{\jbeta}{J_G(\boldsymbol{\beta})}
\newcommand{\Tbeta}{D^2_G(\boldsymbol{\beta})}
\newcommand{\dbeta}{D^3_G(\boldsymbol{\beta})}
\newcommand{\vbeta}{\boldsymbol{v(\beta)}}
\newcommand{\ubeta}{\boldsymbol{u(\beta)}}
\newcommand{\ball}{{\bf B}^p(r)}
\newcommand{\sball}{{\bf B}^p(\boldsymbol\tbeta^{\star},\varepsilon_0)}
\newcommand{\gtbeta}{G(\boldsymbol{\tilde\beta^{\star}})}
\newcommand{\lbeta}{\nabla\ell(\bbeta,\bbZ)}
\newcommand{\kbeta}{\boldsymbol{\beta}_n(k)}
\newcommand{\kkbeta}{\boldsymbol{\beta}_n(k+1)}
\newcommand{\sbeta}{\boldsymbol{\beta}^{\star}}
\newcommand{\tsbeta}{\boldsymbol{\tilde\beta}^{\star}}
\newcommand{\hobeta}{\boldsymbol{\hat\beta}^{\mathcal{O}}}
\newcommand{\thrbeta}{\boldsymbol{\hat\beta}^{thr}}
\newcommand{\pbeta}{\boldsymbol{\pi(\bbeta)}}
\newcommand{\oball}{{\bf B}^p_0(s_0)}
\newcommand{\lball}{{\bf B}^p_1(r_b)}
\newcommand{\bDelta}{\boldsymbol{\Delta}}

\setlength{\headheight}{0in} \setlength{\headsep}{0in}


\title{
Statistical Inference for High-Dimensional Robust Linear Regression Models via Recursive Online-Score Estimation
}
\author{ Dian Zheng and Lingzhou Xue
}

\date{\today}


\renewcommand{\baselinestretch}{1.6}






